Smoothening block rewards: How much should miners pay for mining pools?

The rewards a blockchain miner earns vary with time. Most of the time is spent mining without receiving any rewards, and only occasionally the miner wins a block and earns a reward. Mining pools smoothen the stochastic flow of rewards, and in the ideal case, provide a steady flow of rewards over time. Smooth block rewards allow miners to choose an optimal mining power growth strategy that will result in a higher reward yield for a given investment. We quantify the economic advantage for a given miner of having smooth rewards, and use this to define a maximum percentage of rewards that a miner should be willing to pay for the mining pool services.

==> ensemble.tex <==
\begin{tikzpicture}
    \begin{axis}[
        title={Ensemble vs. Time Average},
        xlabel={Time},
        ylabel={Value},
        xmin=0, xmax=10,
        ymin=0, ymax=5,
        axis lines=center,
        legend pos=north west,
        ytick=\empty,
        xtick={2,8},
        xticklabels={Start,End},
    ]

    % Ensemble average
    \addplot [
        color=blue,
        mark=none,
        ] 
        coordinates {
        (2,2.5)
        (2,4)
        };
    \addplot [
        color=blue,
        mark=none,
        ] 
        coordinates {
        (2,2)
        (2,1)
        };
    \addplot [
        color=blue,
        mark=none,
        ] 
        coordinates {
        (2,3)
        (2,2.5)
        };
        
    % Time average
    \addplot [
        color=red,
        mark=none,
    ]
    coordinates {
    (2,3.5)
    (8,3.5)
    };
    
    \legend{Ensemble Average, Time Average}
    
    \end{axis}
\end{tikzpicture}

==> proof_exp_util.tex <==
\textbf{WIP}\\

\hline
which, for the sake of exposition, we derive next in a slightly more general setting than that of \cite{peters2011time}. Let $W(n)=W_n$ denote the wealth of a player (resp. miner) after $n$ epochs. Furthermore, let $c_n$ (possibly a random variable with known distribution) denote the cost to play (resp. operational expenses) and $\mathcal{M}_n$ denote the rewards from playing (resp. mining) at epoch $n$,  and assume that there exists constants $k$ and $\nu$ such that $c_n=kW_n$ and $\mathcal{M}_n=\nu W_n$. This assumption means that the cost of playing t and the rewards are directly proportional to the wealth of a player (which can hold up reasonably well in the case of mining crypto currencies; large rigs generate more rewards, but also require a larger maintenance and investment cost). From this, given some initial wealth $W_0\in\mathbb{R}_+$, and defining \begin{align}
    r_n:=\frac{W_{n-1}-c_n+\mathcal{M}_n}{W_{n-1}}\\
    =1+\mu-k.
\end{align}
one can then write  $W_T$ as
\begin{align}
    W_T=W_0\prod_{n=1}^Tr_n, \quad \forall T\in\mathbb{N}_+.
\end{align}
Notice that since $\mathcal{M}_n$, and potentially $c_n$, are random variables, so will be $W_n$. Now, assume that  Thus, taking the \textit{time average} of  $W_T$, we obtain
\begin{align}
   \wh:=\lim_{T\to\infty} W_T^{1/T}=W_0\lim_{T\to\infty}\left(\prod_{n=1}^Tr_n\right)^{1/T}.
\end{align}
Now, let $n'$ denote the number of  \textit{coin tosses} (resp. blocks mined in a round), with a maximum of  $N_T$. Notice that the term $\prod_{n=1}^Tr_n$ can be written as 
\begin{align}
\prod_{n=1}^Tr_n&=(\underbrace{r_{i_1}\cdot r_{2_1}\dots \cdot r_{k_1}}_{\text{1 winning block, $k_1$ times}})\times (\underbrace{r_{1_2}\cdot r_{2_2}\dots \cdot r_{k_2}}_{\text{2 winning blocks, $k_2$ times}})\times\dots \times (\underbrace{r_{1_{N_T}}\cdot r_{2_{N_T}}\dots \cdot r_{k_{N_T}} }_{\text{$N_T$ winning blocks, $k_{N_T}$ times}})\\
&=\prod_{n=1}^T r_{n'}^{k_{n'}}
%=
\end{align}
 \textbf{END WIP}\\
 
 \hline
}

==> removed.tex <==
\rjp{
A possible solution to the St. Petersburg paradox was proposed in \cite{peters2011time}, where it was shown that it is wrong to assume the expected reward, which is given by the ensemble average of different payouts, is the relevant quantity to player finances. }

\rjp{In summary, computing an expected payoff as an ensemble average, is equivalent to the assumption that a large number $N$ of identical games are being played in parallel, where they randomly reach different outcomes, The ensemble average corresponds to the average result of all of the games that were played in parallel. The expected value is calculated by letting $N$ go to infinity and averaging over all parallel game outcomes.

In reality when a player is playing the St. Petersburg game, it doesn't matter to the player what would happen in $N$ alternative realities, but what will happen in their one game over time: what is expected to happen to the wealth of that player if they played the game $N$ times in a row? 

This mean that the player is more interested in the ``time-averaged" outcome of the game, where a game is played $N$ times sequentially, than in the ensemble average, where $N$ games are played in parallel one time.

It is a foundational principle of statistical mechanics, to assume that for certain systems that meet certain criteria, the ensemble average and time average are equivalent. Such systems are known as ``ergodic systems".

It has recently been shown in \cite{peters2011time} that for the St. Petersburg paradox, the game is not an ergodic system, and in fact when one examines the time average of the  rewards, the paradox is resolved: there is no longer a non-intuitive infinite reward.}



The relevant quantity proposed in \cite{peters2011time} is the \textit{wealth growth rate}, 
Suppose a player has at $t=0$, an amount of wealth, \ajp{$W_0$}
$$\mathbb{E}\left[W(T)\right]=W_0e^{gT},$$
where $g$ is the expected growth rate, which is the quantity of interest. If $g$ is larger than 0, then the player should accept to play the game, as they would expect that their wealth will grow over time.

As shown in \cite{peters2011time}, the expected growth rate is computed as follows. Suppose playing the game has a set of possible outcomes, labeled by $n$, where the corresponding payout for each outcome is $J_n$, and the cost to the player to play such game is $c_n$ (a constant cost was used in \cite{peters2011time}, but we generalize to the $n$-dependent case, as we will need it for our block reward problem). The probability of outcome $n$ is \ajp{$q_n$}.  The expected time duration of one round of the game is $\bar{t}$ (this is normalized to $\bar{t}=1$ in ref \cite{peters2011time})The expected growth rate is then given by

\begin{eqnarray}
    g=\frac{1}{\bar{t}}\sum_n q_n\log\left(\frac{W_0-c_n+J_n}{W_0}\right).\label{growthrate}
\end{eqnarray}

Playing the game is only rational when $g>0$.



